Stochastic Variational Video Prediction

Predicting the future in real-world settings, particularly from raw sensory observations such as images, is exceptionally challenging. Real-world events can be stochastic and unpredictable, and the high dimensionality and complexity of natural images requires the predictive model to build an intricate understanding of the natural world. Many existing methods tackle this problem by making simplifying assumptions about the environment. One common assumption is that the outcome is deterministic and there is only one plausible future. This can lead to low-quality predictions in real-world settings with stochastic dynamics. In this paper, we develop a stochastic variational video prediction (SV2P) method that predicts a different possible future for each sample of its latent variables. To the best of our knowledge, our model is the first to provide effective stochastic multi-frame prediction for real-world video. We demonstrate the capability of the proposed method in predicting detailed future frames of videos on multiple real-world datasets, both action-free and action-conditioned. We find that our proposed method produces substantially improved video predictions when compared to the same model without stochasticity, and to other stochastic video prediction methods. Our SV2P implementation will be open sourced upon publication.

==> sections___scratch.tex <==
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}

%%SL.10.14: It would be good to start this section with a little bit of motivation before diving into the math

%%SL.10.14: I would recommend that we use $\mathbf{x}_t$ as the tth frame, and $\mathbf{z}_t$ as the tth latent (but first introduce $\mathbf{z}$ as a per-sequence latent).
Let $x$ and $y$ denote the previous and future frames of a video respectively. We assume the whole video $(x,y)$ is generated from a conditional distribution $p(x,y|z)$ where $z$ is a latent variable sampled from a prior distribution $p(z)$. The stochastic video prediction problem is to model $p_\theta(y|x,z)$. Please note that the true posterior $p(z|x,y)$ is intractable since it depends on $p(x,y)$. We overcome this problem by approximating the posterior $q_\phi(z|x,y)$ with family of diagonal Gaussian distributions $\mathcal{N}(\mu, \sigma)$ and using the same reparameterization trick as \VAE~\citep{kingma2013auto}:
%DE10.13: define \theta
%%SL.10.14: I think that it would be better to define the entire probabilistic graphical model. Here is one way we can present the motivation for the model:

In order to construct our stochastic video prediction model, we first formulate a probabilistic graphical model that explains the stochasticity in the video. Since our goal is to perform conditional video prediction, the predictions are conditioned on a set of $c$ \emph{context} frames $\bx_0,\dots,\bx_{c-1}$ (e.g., if we are conditioning on one frame, $c=1$), and our goal is to sample from $p(\bx_c,\dots,\bx_T | \bx_0, \dots, \bx_{c-1})$. Video predictions may be stochastic due to the presence of latent events that are not observed from the context frames alone. For example, when a robot's arm pushes a toy on a table, the unknown weight of that toy might affect how it moves. We therefore introduce a vector of latent variables $\bz$ into our model, distributed according to a prior $\bz \sim p(\bz)$, and build a model $p(\bx_c,\dots,\bx_T | \bx_0, \dots, \bx_{c-1}, \bz)$. This model is still stochastic, but can make use of a much simpler represented, such as a conditional Gaussian, to explain just the noise in the image, since $\bz$ accounts for the more complex stochastic phenomena. We can then factorize this model according to $\prod_{t=c}^T p(\bx_t | \bx_0, \dots, \bx_{t-1}, \bz)$. Learning then involves training the parameters of these factors (which we assume are shared). This requires marginalizing out the latent variable $\bz$.

\begin{align}
\label{eqn:laten_sampling}
&z = \mu_\phi(x,y) + \sigma_\phi(x,y) \times \epsilon, \hspace{1cm} \epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})\\
&y \sim p_\theta(y|x,z) \nonumber
\end{align}


Where $\theta$ and $\phi$ are the parameters of the generative and inference models respectively. This formulation leads to the loss function similar to VAE which can be minimized by SGD:

$$\mathcal{L}(x) = -\E_{q_\phi(z|x,y)}\big[\log p_\theta(y|x,z)\big] + D_{KL}\big(q_\phi(z|x,y)||p(z)\big)$$

Where $D_{KL}$ is the Kullback-Leibler divergence between approximated posterior and assumed prior $p(z)$ which we let to be the standard Gaussian $\stdgauss$. The first term in RHS represents the reconstruction loss while the second term indicates the error of latent approximation. In action-conditioned settings, we modify the generative model to be also conditioned on actions $p(y|x,z,a)$ while keeping the posterior approximation intact.
%%SL.10.14: Should have a separate $\paragraph{...}$ or something for discussing action conditioning

It is important to emphasize that the approximated posterior is conditioned on \textit{\textbf{all}} of the frames, including the ones in the future $y$. This is feasible since $y$ is available at the training time while at the prediction time we can sample the latent from assumed prior rather than the approximated posterior, assuming $D_{KL}\big(q_\phi(z|x)||p(z)\big)~\approx~0$. It is possible to approximate $p(z|x)$ to fix this problem, however, the model would be harder to train in practice because approximating the latent from both past and future frames, is an \textit{easier} task compared to when only the past frames are available. Our experiments support this claim.
%DE10.13: "Our experiments support this claim -- may be worth forward referencing here which experiments do actually support this specific claim.
%%SL.10.14: I think the importance of conditioning on future frames should be articulated more clearly. It's actually crucial to the success of the method. How about this phrasing:
%While we could train an inference network of the form $p(\bz | \bx_{0:t})$ for time step $t$, the model would have little incentive to use $\bz$ to make stochastic predictions in this case, since $\bz$ does not tell the model anything at training time that it does not already know from the past frames $\bx_{0:t}$.

%%SL.10.14: do you want to discuss the per-step model somewhere that uses $\bz_t$?

\subsection{Model Architecture}

To model the approximated posterior $q_\phi(z|x,y)$ we use a deep convolutional neural network, called a \textit{latent tower}, as shown in Figure~\ref{fig:model}. This tower outputs the mean and standard deviation of the approximated posterior, which are $8{\times}8$ single channel images.
%%SL.10.14: I think explaining that the latents are a convolutional response map is alone quite complex and deserves more exposition and discussion
The latent value is then sampled using Equation~\ref{eqn:laten_sampling}.

For the generative model
%%SL.10.14: use the symbol: $p(\bx_t | \bx_0, \dots, \bx_{t-1}, \bz)$
we used the CDNA architecture proposed by~\citet{finn2016unsupervised}, which is a deterministic recurrent neural network that predicts the next frame $I_t$ given the previous frame $I_{t-1}$ and action.
%%SL.10.14: There is a little nuance here: technically, in the VAE framework, this model still makes "stochastic" predictions, but they are very naive: the output loss of mean squared error corresponds to a conditional independent Gaussian over the pixels. Maybe this can be discussed somehow? Else it is weird that a factor p(x_t|...) is represented by a deterministic network.
This model constructs the next frames by predicting the motions of different segments of the image (i.e., objects) and then merging these predictions via masking. Since the model is not aiming to reconstruct the appearance of the objects directly,
%%SL.10.14: This nuance probably deserves more discussion, since the model *does* output pixels. Readers might misunderstand this...
it is partially-appearance invariant and can generalize to unseen objects. To condition the prediction on the latent value, we slightly modify its architecture to accept the latent value next to actions.
%%SL.10.14: kind of funny to say this but then not state how you modify, maybe refer to the section where this is discussed?

\subsection{Training Procedure}

This model can be trained end-to-end. However, our experiments show that a na\"ive training usually results in the model ignoring the latent variables and converging to a suboptimal deterministic solution. Therefore, we train the model end-to-end in three phases, as follows:

\begin{enumerate}%[wide, labelindent=10pt]
\item \textbf{Training generative tower:} In this phase, the latent tower has been disabled and the latent value $z$ will be randomly sampled from $\stdgauss$. The intuition behind this phase is to train the generative model to predict the future frames deterministically (i.e. modeling $p_\theta(y|x)$).
%%SL.10.14: It's not really clear why this is needed.

\item \textbf{Training latent tower:} In the second phase, the latent tower will be trained to estimate the posterior approximation $q_\phi(z|x,y)$, however, the KL-loss will be set to 0. This means that the model can use the latent value without being penalized for diverging from the assumed prior. As it can be seen in Figure~\ref{fig:training}, this phase results in very low reconstruction error, however it is not usable at the testing time since $D_{KL}\big(q_\phi(z|x)||p(z)\big)\gg 0$ and sampling $z$ from assumed prior will be inaccurate.
%%SL.10.14: This makes perfect sense. Maybe tighten the discussion a bit (some minor grammatical/non-idiomatic phrasing)

\item \textbf{Divergence reduction:} In the last phase, the KL-loss will be added to the overall cost, resulting in a sudden drop of divergence loss and an increase of reconstruction error. Reconstruction loss converging to a value lower than the first phase and KL-loss converging to zero are excellent indicators for a successful training. 
\end{enumerate}
%%SL.10.14: it would be good to make clear what the benefit of this is (to make sure we actually train the right model, and so that we can sample $\bz$ at test time and get reasonable stochastic samples)

To gradually transit from the second phase to the third, we add a multiplier to KL-loss which will be set to zero during the first two phases and then will be increased slowly in the last phase. Our experiments show that this training procedure is quite stable and the model converges to the desired parameters almost every time. Since the generative model is predicting the frames one by one, it is possible to sample $z$ once (for the whole video) or per frame. Experiments show that while both models work in practice, multiple sampling generalizes beyond the training data better than the single sampling (cf.~Figure~\ref{fig:graph}). 
%%SL.10.14: I think the multiple sampling model should be first discussed separately in the modeling section


==> sections_prelim.tex <==
\subsection{Variational Autoencoders}
\label{subsec:vae}

\VAE~\citep{kingma2013auto,mnih2014neural} generalizes the original \AE~\citep{vincent2010stacked} by imposing a prior over the latent distribution $p(z)$. Similar to \AE, \VAE ~consists of two networks: an \textit{encoder} that encodes a data sample $x$ from data space to a latent representation $z$ and a \textit{decoder} which decodes $z$ back to the original data space:
$$z \sim q(z|x) = \mathbf{enc}(x), \hspace{1cm} \hat{x} \sim p(x|z) = \mathbf{dec}(x)$$

VAE cost function is the negative sum of the reconstruction error (expected log likelihood) and a prior regularization term which is usually the Kullback-Leibler divergence between the estimated and assumed prior:

$$\mathcal{L}(x) = -\E_{q(z|x)}\big[\log p(x|z)\big] + D_{KL}\big(q(z|x)||p(z)\big)$$

Typically it is assumed that $p(z) \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$. In order to make the model trainable via SGD and therefore differentiable a ``reparameterization trick" is used in which the encoder network estimates the mean $\mu(x)$ and covariance $\Sigma(x)$ of the distribution:

$$z = \mu(x) + \Sigma^{1/2}(x) \times \epsilon, \hspace{1cm} \epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$$


\subsection{Prediction via Flow}
\label{subsec:flow}
The core of motion-focused predictive models~\citep{finn2016unsupervised} is a motion prediction model that predicts the motion of the objects in the image without reconstructing their appearances. In other words, this model constructs the next frames by predicting the motions of different segments of the image (i.e. objects) and then merging these predictions via masking. Since the model is not trying to reconstruct the appearance of the objects directly, it's partially-appearance invariant and can generalize to unseen objects. 
